A primary electron beam facility at CERN -- eSPS Conceptual design report

The design of a primary electron beam facility at CERN is described. The study has been carried out within the framework of the wider Physics Beyond Colliders study. It re-enables the Super Proton Synchrotron (SPS) as an electron accelerator, and leverages the development invested in Compact Linear Collider (CLIC) technology for its injector and as an accelerator research and development infrastructure. The facility would be relevant for several of the key priorities in the 2020 update of the European Strategy for Particle Physics, such as an electron-positron Higgs factory, accelerator R\&D, dark sector physics, and neutrino physics. In addition, it could serve experiments in nuclear physics. The electron beam delivered by this facility would provide access to light dark matter production significantly beyond the targets predicted by a thermal dark matter origin, and for natures of dark matter particles that are not accessible by direct detection experiments. It would also enable electro-nuclear measurements crucial for precise modelling the energy dependence of neutrino-nucleus interactions, which is needed to precisely measure neutrino oscillations as a function of energy. The implementation of the facility is the natural next step in the development of X-band high-gradient acceleration technology, a key technology for compact and cost-effective electron/positron linacs. It would also become the only facility with multi-GeV drive bunches and truly independent electron witness bunches for plasma wakefield acceleration. A second phase capable to deliver positron witness bunches would make it a complete facility for plasma wakefield collider studies. [...]

==> include/00-Preamble/abstract.tex <==

%\end{comment}
%\newpage
%\begin{abstract}
In this Expression of Interest, we propose a primary electron beam facility with the main motivations being (i) dark sector experiments, and (ii) to enable a suite of development projects in acceleration technology. 
We also present a detailed description of an experiment, the Light Dark Matter eXperiment, LDMX, which could make use of this facility to probe thermal dark matter over a majority of the viable sub-GeV mass range. We show that LDMX can achieve orders of magnitude more sensitivity than any previous or currently envisioned experiment. LDMX uses missing momentum to search for dark matter produced via {\it dark bremsstrahlung} produced in the interaction of electrons on a thin target. This requires a low-current, high repetition rate electron beam, with optimal energy of $\sim 16~$\GeV. We propose to create this electron beam at CERN by restoring the SPS's electron acceleration capability. 
%Such a restoration would also provide CERN with completely new possibilities for accelerator project development and for general accelerator R\&D.

%; injecting electrons into the SPS using an X-band 3.5~\GeV~linear electron accelerator constructed in the TT4 transfer tunnel, and slowly extracting a 16~\GeV~beam from the SPS into an experimental area.


%\end{abstract}

==> include/00-Preamble/authors.tex <==
%\author{Name list of people expressing their interest}

%\begin{comment}

\author{Torsten Åkesson}
\affiliation{Lund University, Department of Physics, Box 118, 221 00 Lund, Sweden}

\author{Fanouria Antoniou}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Pablo A. Arrutia Sota}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}
\affiliation{Royal Holloway, University of London, Egham TW20 0EX, UK}

\author{Fabio Bossi}
\affiliation{INFN Laboratori Nazionali di Frascati, Italy}

\author{Antonio Boveia}
\affiliation{The Ohio State University, Department of Physics and Center for Cosmology and Astroparticle Physics, 191 W. Woodruff Ave., Columbus, Ohio 43210, USA}

\author{Markus Brugger}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Lene Bryngemark}
\affiliation{Lund University, Department of Physics, Box 118, 221 00 Lund, Sweden}

\author{Philip N. Burrows}
\affiliation{University of Oxford, Oxford, United Kingdom}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Massimo Carpinelli}
\affiliation{Chemistry and Pharmacy Department, Università degli Studi di Sassari, Sassari 07100, Italy}
\affiliation{INFN Laboratori Nazionali del Sud, Catania 95123, Italy}

\author{Nuria Catalan}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Riccardo Catena}
\affiliation{Chalmers University of Technology, Department of Physics, SE-412 96 G\"oteborg, Sweden}

\author{Augusto Ceccucci}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{James Chappell}
\affiliation{University College London, Gower Street, LONDON, WC1E 6BT, UK}

\author{Owen Colegrove}
\affiliation{University of California at Santa Barbara, Santa Barbara, CA 93106, USA}

\author{Giulia Collura}
\affiliation{University of California at Santa Barbara, Santa Barbara, CA 93106, USA}

\author{Jan Conrad}
\affiliation{Oskar Klein Centre for Cosmoparticle Physics, Fysikum, Stockholm University, 10961 Stockholm, Sweden}

\author{Karel Cornelis}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Roberto Corsini}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Hans Danielsson}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Dominik Dannheim}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Steffen Doebert}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Caterina Doglioni}
\affiliation{Lund University, Department of Physics, Box 118, 221 00 Lund, Sweden}

\author{E. C. Dukes }
\affiliation{University of Virginia, Charlottesville, VA 22904, USA}

\author{Yann Dutheil}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Valentina Dutta}
\affiliation{University of California at Santa Barbara, Santa Barbara, CA 93106, USA}

\author{Bertrand Echenard}
\affiliation{California Institute of Technology, Pasadena, CA 91125, USA}

\author{Ozgur Etisken}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}
\affiliation{Ankara University, Faculty of Sciences, Department of Physics, Turkey}

\author{Lyn Evans}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Matthew A. Fraser}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Alexander Friedland}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}

\author{Jonathan Gall}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Jake S. Gessner}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Brennan Goddard}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Norman Graf}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}

\author{R. C. Group }
\affiliation{University of Virginia, Charlottesville, VA 22904, USA}

\author{Alexej Grudiev}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Edda Gschwendtner}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Vincent Hedberg}
\affiliation{Lund University, Department of Physics, Box 118, 221 00 Lund, Sweden}

\author{Joshua Hiltbrand}
\affiliation{University of Minnesota, Minneapolis, MN 55455, USA}

\author{David Hitlin}
\affiliation{California Institute of Technology, Pasadena, CA 91125, USA}

\author{Joseph Incandela}
\affiliation{University of California at Santa Barbara, Santa Barbara, CA 93106, USA}

\author{Lars Jensen}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Robert Johnson}
\affiliation{Santa Cruz Institute for Particle Physics, University of California at Santa Cruz, Santa Cruz, CA 95064, USA}

\author{Rhodri Jones}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Venelin Kozhuharov}
\affiliation{Sofia University, Bulgaria}

\author{Gordan Krnjaic}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL 60510, USA}

\author{Mike Lamont}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Andrea Latina}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Thibaut Lefevre}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Emanuele Leonora}
\affiliation{INFN- Sezione di Catania, Italy}

\author{Lucie Linssen}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Fabio Longhitano}
\affiliation{INFN- Sezione di Catania, Italy}

\author{Olle Lundh}
\affiliation{Lund University, Department of Physics, Box 118, 221 00 Lund, Sweden}

\author{Else Lytken}
\affiliation{Lund University, Department of Physics, Box 118, 221 00 Lund, Sweden}

\author{Jeremiah Mans}
\affiliation{University of Minnesota, Minneapolis, MN 55455, USA}

\author{Takashi Maruyama}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}

\author{Jeremy McCormick}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}

\author{Gerard Mcmonagle}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Eric Montesinos}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Omar Moreno}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}

\author{Patric Muggli}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Geoffrey Mullier}
\affiliation{Lund University, Department of Physics, Box 118, 221 00 Lund, Sweden}

\author{Timothy Nelson}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}

\author{Gavin Niendorf}
\affiliation{University of California at Santa Barbara, Santa Barbara, CA 93106, USA}

\author{John A. Osborne}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Yannis Papaphilippou}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Reese Petersen}
\affiliation{University of Minnesota, Minneapolis, MN 55455, USA}

\author{Ruth Pöttgen}
\affiliation{Lund University, Department of Physics, Box 118, 221 00 Lund, Sweden}

\author{Javier Prieto}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Mauro Raggi}
\affiliation{Dipartimento di Fisica, Sapienza Università di Roma and INFN Roma, Italy}

\author{Nunzio Randazzo}
\affiliation{INFN- Sezione di Catania, Italy}

\author{Alexander Read}
\affiliation{Department of Physics, University of Oslo, Postbox 1048, 0316 Oslo, Norway}

\author{Philipp Roloff}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Carlo Rossi}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Andre Sailer}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Daniel Schulte}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Philip Schuster}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\affiliation{Perimeter Institute for Theoretical Physics, Waterloo ON N2L 2Y5, Canada}

\author{Eva Sicking}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Valeria Sipala}
\affiliation{Chemistry and Pharmacy Department, Università degli Studi di Sassari, Sassari 07100, Italy}
\affiliation{INFN Laboratori Nazionali del Sud, Catania 95123, Italy}

\author{Steinar Stapnes}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Igor Syratchev}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}

\author{Natalia Toro}
\affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\affiliation{Perimeter Institute for Theoretical Physics, Waterloo ON N2L 2Y5, Canada}

\author{Nhan Tran}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL 60510, USA}

\author{Domenico D'Urso}
\affiliation{Chemistry and Pharmacy Department, Università degli Studi di Sassari, Sassari 07100, Italy}
\affiliation{INFN Laboratori Nazionali del Sud, Catania 95123, Italy}

\author{Paolo Valente}
\affiliation{INFN Roma, Italy}

\author{Andrew Whitbeck}
\affiliation{Fermi National Accelerator Laboratory, Batavia, IL 60510, USA}

\author{Walter Wuensch}
\affiliation{CERN, CH-1211 Geneva 23, Switzerland}




==> include/05-ICE/OLD_CDR_Text.tex <==
%This file contains all of the stuff from the old CDR section layout -- Copy and paste into new structure
%%Contents of old stuff
% Civil engineering
%cooling and ventilation
%Electrical instillation
% Integration 
%Radiation studies and protection
%safety
%transport



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% COOLING AND VENTILATION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Cooling and Ventilation} \label{sec:ICE_CnV}

The Cooling and Ventilation section is composed of three parts. The first regards piped utilities, the second outlines the air-related systems and the third addresses safety and environmental protection.

The design herewith presented is based on the latest user requirements. A safety margin of approximately 15\% was applied to the heat loads, given the early stage of the project. Additionally, the infrastructure was designed to be flexible and allow for future upgrades and extensions. Energy consumption is considered a priority and different strategies, as the use of air economizers, are adopted to increase the overall efficiency. 

\subsubsection{Piped Utilities} \label{sec:Piped Utilities}

The piped utilities are mainly dedicated to the cooling of the accelerator equipment and the related infrastructure such as power converters, electronic racks, cables, etc..., as well as to the ventilation and air-conditioning of underground and surface premises. In addition, specific systems are foreseen to cover other general needs such as fire extinguishing plants, drainage and sumps (for both surface and underground areas), drinking water and compressed air for ancillary equipment (vacuum pumps, valves, dampers, etc.). The main circuit typologies are list below:

\begin{itemize}
\item Industrial and demineralized water: for the cooling of accelerator equipment (ex.: magnets, accelerating cavities, power converters, etc.) and infrastructure (water cooled cables, chillers, etc.);
\item Chilled water: at present, used exclusively in ventilation and air-conditioning plants;
\item Industrial water for firefighting systems: industrial water circuits are in place to assist firefighters in case of fire;
\item Wastewater: water from underground and surface premises that is to be rejected ;
\item Drinking water: for sanitary purposes, make up of industrial water circuits and production of demineralized water;
\item Industrial water for firefighting systems;
\item Compressed air: mainly for ancillary equipment as pneumatic valves or vacuum pumps.
\end{itemize}

Two different typologies of water cooling circuits are defined according to their equipment and working temperatures: demineralized water circuits and chilled water ones. The first are cooled by primary circuits (industrial water) and the latter by chillers, that are able produce water at lower temperatures, as portrayed in Fig. \ref{fig:cvcircuits}.

The primary water circuits, cooled by open wet cooling towers, are configured in closed loops to minimize water consumption. Drinking water is used to compensate for evaporation, leaks and blowdown. A continuous water treatment against legionellae, scaling and proliferation of algae is foreseen.

Generally, demineralized water circuits are used to refrigerate equipment and have a maximum conductivity of 0.5 $\mu$S/cm. A set of demineralization cartridges is foreseen for each circuit, in order to locally control the conductivity. The leaving temperature is controlled to be 27 \si{\degree}C ($\pm0.5$ \si{\degree}C).

Chilled water is employed to condition air at air-handling units. If dehumidification is required, the leaving water temperature is typically 6 \si{\degree}C, otherwise it is usually raised to values of around 14 \si{\degree}C.
The design temperature differences for chilled water and demineralized water circuits is of 6 \si{\degree}C and 8 \si{\degree}C respectively, as one can verify in Fig. \ref{fig:cvcircuits}.

\begin{figure}[t!]
\begin{center}
    \includegraphics[width=10cm]{include/05-ICE/Figures/CVCircuits.pdf}
    \caption{Two typologies of cooling circuits}
 \label{fig:cvcircuits}
\end{center}
\end{figure}


DETAILS OF THE COOLING


Most electromechanical cooling components, as cooling towers, pumps and chillers have N+1 redundancy. On the other hand, no redundancy is foreseen for electrical cubicles, control cubicles and heat exchangers. Under present conditions, there is no need to provide a secure power supply for the majority of the cooling plants. In case of power failure, all accelerator related equipment stop and do not require any cooling. Chilled water pumps for critical ventilation systems are an exception and do have a secured power supply. They will circulate water stored in buffer tanks (the chillers are off in case of electrical failure) that are designed to provide sufficient autonomy. The power supply for the PLCs within the control cubicles are protected by batteries to ensure proper shutdown and avoid losing the control program.

The drinking water network is used for sanitary purposes and as make-up water for the cooling towers. The existing drinking water network at CERN is extended and upgraded to satisfy the new requirements.

The existent firefighting water network is modified to ensure the safety of personnel and equipment. Fire hydrants are foreseen at external areas, while flexible hoses are foreseen inside the premises. Pipelines running in underground facilities, as the LINAC tunnel or the detectors cavern will be kept dry to avoid corrosion and stagnation. In case of fire, the fire brigade will open manual valves at the surface to supply water to the concerned area.

The reject water is split in two distinct networks - one for clear waters and one for sewage; these networks are connected to the corresponding existing systems at each area.
For safety reasons each sump will be equipped with sensors providing alarms for high and too high level; in addition, pumps in the underground sumps will be redundant.
Thorough control mechanisms are implemented before releasing reject water to existing natural water lines. Relevant parameters such as pH and temperature are monitored and corresponding alarms implemented; if the quality of the water does not comply with the required level, retention basins and other measures will be taken to improve the quality before discharge.
A new process to concentrate the chemicals in the cooling towers blowdown water is presently being studied at CERN. We expect to implement this system in future cooling plants. As a consequence, this water is rejected to the sewage line.

The needs and requirements for compressed air are not been defined at this stage of the project; however, existing networks are present along CERN premises. If their capacity is not sufficient, or if the existing lines cannot be used (for any other reason), new production stations will be installed. An N+1 redundancy is foreseen for the compressors at each station.

\subsubsection{Heating Ventilation and Air-Conditioning} \label{sec:Heating Ventilation and Air-Conditioning}

The heating, ventilation and air conditioning plants are designed to:

\begin{itemize}
\item Supply fresh air to people;
\item Filter the supply and exhaust air
\item Sustain a given temperature and/or humidity in each area;
\item Extract smoke and gas if necessary;
\item Purge the tunnels if necessary.
\end{itemize}

The indoor conditions are summarized in the following table.

\begin{table}[!h]
\begin{center}
\caption{Indoor Conditions}
\label{tab:IndoorConditions}
\begin{tabular}{p{6cm}cc}
\hline\hline
\textbf{Component}          	& \textbf{Ambient T}   	& \textbf{Particular Requirements [\%]}\\
\hline
LINAC Tunnel                    & Y           				& 4.5 \\
Klystron Gallery                & Y             			& 2.3 \\
Detectors Building              & Y                         & 2.2 \\
Surface Buildings               & Y                			& 0.3 \\
\hline\hline
\end{tabular}
\end{center}
\end{table}


\subsubsection{Safety and Environmental Protection} \label{sec:Safety and Environment Protection}

use of chilled water is minimized. Using cooling towers as the heat sink is significantly...

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ELECTICAL INSTALLATION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Electrical Installations}
\label{sec:ICE_EL}

To be written by Davide and Carlo

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Integration %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Integration}
\label{sec:ICE_Integration}

To be written by Liam

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Radiation studies and protection %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Radiation Studies and Protection}
\label{sec:ICE_Radiation}

To be written by Markus W.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Safety %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Safety and Access Control}
\label{sec:ICE_Safety}

To be written by Owain and Simon

\subsubsection{Introduction} \label{Sec:Introduction}

In all of the technical considerations for a facility such as BDF, it is essential to consider safety and environmental protection as an integral part of the comprehensive design, taking conscious decisions early-on to eliminate or significantly reduce potential hazards, in a cost-effective, pragmatic manner.

\subsubsection{Legal context of CERN} \label{Sec:Legal}

By virtue of its intergovernmental status, CERN is entitled to adopt its own internal organisational rules, which prevail over national laws to facilitate the execution of its mission. In the absence of specific CERN regulations, the laws and regulations of the Host States generally prevail.

In response to its unique geographical situation (straddling without discontinuity across the Swiss-French border) and its highly specific technical needs, the Organization stipulates its safety policy, in the frame of which it establishes and updates rules aimed to ensure uniform safety conditions across its sites. CERN's safety rules apply to the Organization's activities, as well as to persons participating in CERN's activities or present on its site. 

When establishing its own safety rules, CERN takes into account the laws and regulations of the Host States, EU regulations and directives as well as international regulations, standards and directives and, as a general principle, CERN aligns with these as much as reasonably possible. 

Where such compliance is not possible or desirable due to technical or organisational constraints, such as for equipment and facilities not covered by normal standards, specific clearance from CERN's Occupational Health \& Safety and Environmental Protection Unit (HSE Unit)
based on a risk assessment and compensatory measures is required.

\subsubsection{Occupational Health and Safety} \label{Sec:OH&S}

CERN's Safety Policy, in order of priority, sets out to protect all persons affected by its activities, to limit the impact of the Organization's activities on the environment, and to protect its equipment and ensure continuity of operations. 
The agreed safety objectives are shown in Table~\ref{Tab:Safety:AgreedObjectives}:

\begin{table}[htbp]
\centering
\caption{\label{Tab:Safety:AgreedObjectives} Agreed safety objectives for the BDF project}
\smallskip
\begin{tabular}{|c|c|c|c|c|} 
\hline
\textbf{} & \textbf{A: Life Safety} & \textbf{B: Environmental Protection} & \textbf{C: Property \newline Protection} & \textbf{D: Continuity of Operation}\\
\hline
 1 & Safe evacuation of valid occupants & Limited release of pollutants to air & Continuity of \newline essential services & Limit downtime \\ \hline
 2 & Safe evacuation or staging of injured occupants & Limited release of pollutants to water & Incident shall not cause further \newline incidents &  \\ 
\hline
 3 & Safe intervention of rescue teams &  & Limit property loss &  \\ 
\hline
\end{tabular}
\end{table}

\subsubsection{Fire safety} \label{Sec:Fire}

The goal of fire safety is to protect occupants, rescuers, the external population, the environment, the facility itself, and continuity of operation. To this end, all buildings, experimental facilities, equipment and experiments installed at CERN shall comply with CERN Safety Code E. In view of the special nature of the use of certain areas, in particular underground, with increased fire risk, the HSE Unit is to be considered the authority of approving and stipulating special provisions.  

As the project moves to the Technical Design Report stage, finalising layouts and interconnecting ventilation systems, detailed fire risk assessments will have to be made for all areas of the BDF complex, i.e., Extraction Tunnel, Target Complex and Experimental Hall. At this stage, a general fire safety strategy has been produced, based upon the location and current level of design, along with the latest fire safety strategies employed at CERN. The complex will be considered as an extension of the fire concept developed for the whole of the North Area \cite{NorthArea_FireRA}. 

The most efficient protection strategy is one that uses multi-level "safety barriers", with a bottom-up structure, to limit fires at the earliest stages with the lowest consequences, thus considerably limiting the probability and impact of the largest events. 

In order to ensure that large adverse events are possible only in very unlikely cases of failure of many barriers, measures at every possible level of functional design need to be implemented: 

\begin{itemize}
\item in the conception of every piece of equipment (e.g. materials used in electrical components, circuit breakers, etc.); 
\item in the grouping of equipment in racks or boxes (e.g. generous cooling of racks, use of fire-retardant cables, and fire detection with power cut-off within each rack, etc.); 
\item in the creation and organisation of internal rooms (e.g., fire detection, power cut-off and fire suppression inside a room with equipment); 
\item in the definition of fire compartments; 
\item in the definition of firefighting measures. 
\end{itemize}

The key fire safety strategy concepts can be split into compartmentalisation, fire detection, smoke extraction and fire suppression, as set out below.

\paragraph{Compartmentalisation}

Compartmentalisation impedes the propagation of fire and potentially activated smoke through a facility, allowing occupants to escape to a comparatively safe area much more quickly than otherwise, as well as facilitating the effective fighting of the fire, and evacuation of victims by the Fire Brigade. In the North Area fire concept, the following requirements have been set:

\begin{itemize}
\item All ventilation doors must be fire doors EI90;
\item Isolate communicating galleries with fire doors EI90; 
\item Isolate neighbouring surface facilities with fire doors EI120;
\item Avoid compartments longer than 450m;
\item Normally opened fire doors to be equipped with remote action release mechanism, monitoring position and self-action thermal fuse. 
\end{itemize}

\subparagraph{Extraction Tunnel}

The fire doors will follow the standard requirements for the North Area Fire Concept: 0.9 m minimum width, with fire doors EI90 or greater. They will be set to a normally-closed configuration, due to the ventilation specification and needs of the Extraction Tunnel. The door separating the Extraction Tunnel from the SPS shall be EI120.

\subparagraph{Extraction Tunnel}
The following areas shall be divided into separate fire compartments (shown in Figure \ref{fig:BDF_complex}):

\begin{itemize}
\item Auxiliary Building;
\item Access Building;
\item Target Building;
\item Lower Target Building;
\item Surface Hall;
\item Experimental Hall.
\end{itemize}

It is to be noted that both the Experimental Hall and the Lower Target Building shall be separate compartments from the corresponding Surface Hall and Target Building, accounting for the differing uses of the spaces. The Lower Target Building shall also be divided into several separate fire compartments, corresponding to the pressure cascades implemented for radiation containment.


\paragraph{Fire Detection}

An early fire detection system, integrated into the safety action system is a crucial component of the North Area fire strategy. Early detection is such that allows evacuation (last occupant out) before untenable conditions are reached; the CERN HSE Fire Safety team shall be consulted for this design. The system must be capable of transmitting an alarm, along with a message containing safety instructions, to occupants anywhere in the North Area. This alarm shall be triggered upon fire detection, action on evacuation push buttons, CERN Fire Brigade action out of CERN FB SCR/CCC or BIW (Beam Imminent Warning) situations. Evacuation push buttons shall cover all premises. The fire detection and evacuation push buttons must also be integrated with safety actions such as compartmentalisation, ventilation stop and other machine functions according to a predefined fire protection logic.
Fire detection encompasses the following actions: 

\begin{itemize}
\item Close all fire doors in the fire compartment of origin and the adjacent fire compartments;
\item Trigger an evacuation alarm in the fire compartment of origin and the adjacent fire compartments;
\item Stop free-cooling ventilation; 
\item Broadcast an information message through the public address system; 
\item Trigger a level 3 alarm in the CSAM system, which alerts the CERN Fire Brigade control room, and results in crews being dispatched immediately.
\end{itemize}

\paragraph{Smoke Extraction}
An additional consideration for fires in accelerator tunnels is the danger of potentially activated smoke, and the need to handle this in a controlled manner to limit the release of polluting agents to the environment. A fire assessment methodology that entails the radiological hazard induced by a fire event is currently under development by the FIRIA Project led by HSE. Many of the concepts featured in the FIRIA methodology have been incorporated in the safety support provided by HSE to the BDF project. However, once the FIRIA Methodology is fully available in July 2021, it is recommended to consider carrying out a FIRIA exercise as part of the Technical Design Report phase.
A description of the FIRIA project is available in \cite{FIRIA_Kickoff}.  


\subparagraph{TT61}


\paragraph{Fire Suppression}
 The CERN Fire Brigade need adequate means of fighting a fire on arrival, including a surface hydrant network, which shall be foreseen as the project moves to the Technical Design Report stage, in tandem with the HSE Fire Safety specialists.
 
 \subparagraph{}{TT61}
Dry Risers shall be installed throughout the underground areas, allowing the CERN Fire Brigade to choose to supply water to them for firefighting as required. The additional fire loads and radiation risks present in the Lower Target Building require the addition of a suppression system, to be specified in detail as the project moves into the Technical Design Report phase. A number of fire suppression solutions for such challenging environments are being considered at CERN, such as the delivery of fire suppression by remotely operated drones, which may be applied in this area.


\subsubsection{Safety of Civil Structures} \label{Sec:Civil}


\subsubsection{Chemical Safety} \label{Sec:Chemical}

\subsubsection{Electrical Safety} \label{Sec:Electrical}
The electrical infrastructure design for the BDF facility is currently at a general level, but will incorporate subsystems that either produce, or use, high voltage or current, both of which represent electrical hazards to personnel. Dedicated electrical rooms will be used to contain all the electrical cabinets required for the power distribution. The hazards are expected to be standard for such an installation, and shall be mitigated through sound design practice and execution. The CERN Electrical Safety rules, alongside NF C 18-510, shall be followed throughout the design process; where exceptions are required, this shall be subject to an appropriate level of risk assessment to evaluate the residual risk, and determine the mitigation strategies required. NF C 18-510 compliant covers, interlocks preventing access to high voltage equipment, and restriction of access to the electrical rooms to those with the appropriate level of CERN electrical \textit{habilitation} training shall be used to protect personnel from any electrical hazards present.

\paragraph{Electromagnets}
Of particular interest from an electrical safety perspective will be the magnetic coil and steel yoke, located downstream of the Target. This is likely to be the highest voltage component in the system. As for all electromagnets, appropriate grounding measures shall be implemented for the magnet yokes, and all live parts protected to a minimum of IPXXB for Low Voltage and IPXXC for High Voltage circuits or locked out for any intervention in their vicinity. Interventions may only be carried out by personnel with the necessary training, after following the work organisation procedures and authorisation of the facility coordinator (VICs, IMPACT etc.).

\subsubsection{Mechanical safety and design of the Target Complex} \label{Sec:Mechanical}
The cooling requirements of the target due to the high energy levels being deposited by the beam, along with the high radiological activation levels of the materials surrounding the target have led to the need for a number of different pressurised fluid circuits within the Target Complex.

\noindent All pressure equipment shall comply with the following CERN Safety rules:

\begin{itemize}
    \item CERN Safety Regulation SR-M - Mechanical equipment;
    \item CERN General Safety Instruction GSI-M-2 - Standard Pressure Equipment.
\end{itemize}

Moreover, there are specific sets of rules applicable only to certain types of standard pressure equipment. Those rules are defined in the following Specific Safety Instructions, of which the following may be applicable to the BDF project:

\begin{itemize}
    \item CERN Specific Safety Instruction on pressure vessels (SSI-M-2-1);
    \item CERN Specific Safety Instruction on safety accessories for standard pressure equipment (SSI-M-2-3);
    \item CERN Specific Safety Instruction on metallic pressurised piping (SSI-M-2-4);
    \item CERN Specific Safety Instruction on vacuum chambers and beam pipes (SSI-M-2-5);
    \item CERN Specific Safety Instruction on transportable pressure equipment (SSI-M-2-6).
\end{itemize}

According to CERN Safety rules, pressure equipment shall meet the essential requirements set by the following applicable European Directives:

\begin{itemize}
    \item Directive 2014/68/EU on pressure equipment - Pressure Equipment Directive (PED);
    \item Directive 2010/35/EU on transportable pressure equipment - Transportable Pressure Equipment Directive (TPED).
\end{itemize}

Pressure equipment designed and manufactured according to harmonised European standards benefit from presumption of conformity with the essential requirements laid down in the above mentioned European Directives. In accordance with the CERN Safety rules, the use of harmonised European standards is compulsory for pressure equipment designed and/or manufactured at CERN. The use of other design codes or national standards shall be reviewed and approved by the HSE Unit.

\subsubsection{Non-Ionising Radiation}
The high magnetic fields from the proposed electromagnets in the current BDF design represent a hazard similar to that found in many of the facilities at CERN, and shall be handled with standard mitigation strategies. The facility shall follow the Directive 2013/35/EU on the occupational exposure of workers, alongside CERN Safety Instruction IS 36 and its Amendment. Any activity inside the static magnetic field shall be subject to risk assessment and ALARA. Personnel shall be informed about the hazards and appropriately trained. Areas with magnetic flux densities exceeding 0.5 mT shall be delimited (use pacemaker warning signs), while areas with magnetic flux densities exceeding 10 mT shall be rendered inaccessible to the public. 

\paragraph{Extraction Tunnel}
Electromagnets are foreseen in the BDF extraction beam line, with modified splitter magnets, quadrupoles, dilution kickers and dipole magnets present in the optics design, all of which are to be largely identical to those already in use in the North Area. All magnets foreseen for the facility are warm magnets.

\subsubsection{Noise}
The BDF facilities are located in the North area of the Prévessin site, close to the fence line of CERN property. In order to ensure occupational health and safety to people exposed to noise, the BDF project shall be compliant with the following rules and Regulations:

\begin{itemize}
    \item CERN Safety Code A8 - Protection against noise
    \item Directive 2003/10/EC of the European Parliament and of the Council of 6 February 2003 on the minimum health and safety requirements regarding the exposure of workers to the risks arising from physical agents (noise)
    \item French Code du travail
\end{itemize}
    
\noindent Emissions of environmental noise related to neighbourhoods shall respect the thresholds indicated in:
    
\begin{itemize}    
    \item \textit{French Arrêté du 23 janvier 1997 relatif à la limitation des bruits émis dans l'environnement par les installations classées pour la protection de l'environnement.}
\end{itemize}

\subsubsection{Asbestos}
As the extraction tunnel was constructed before 1997, an asbestos survey was carried out by HSE Unit. The findings of the investigation are summarised in EDMS 2054048.
In case the presence of asbestos is ascertained, necessary protective measures have to be put in place following the applicable CERN Safety rule:

\begin{itemize}    
    \item Safety Instruction IS 43 - Asbestos : Dangers and precautions
\end{itemize}


\subsubsection{Protection of the environment}

\noindent With regard to protection of the environment, CERN Safety Policy states that the Organization is committed to ensuring the best possible protection of the environment. This can be achieved by ensuring that the given regulations are followed for the different activities and experiments. 

As the project moves to the Technical Design Report stage, a review with the Environmental Protection specialists within HSE shall be held to determine whether the relevant technical provisions of the following regulation shall apply for the BDF project:

\begin{itemize}    
    \item \textit{Arrêté du 29/05/00 relatif aux prescriptions générales applicables aux installations classées pour la protection de l'environnement soumises à déclaration sous la rubrique no 2925;}
    \item \textit{Arrêté du 14/12/13 relatif aux prescriptions générales applicables aux installations relevant du régime de l'enregistrement au titre de la rubrique no 2921 de la nomenclature des installations classées pour la protection de l'environnement.}
\end{itemize}

\noindent The technical environmental mitigation measures shall be determined more precisely once technical detail information are available such as the type and the quantity of chemicals or the solution chosen for the cooling. 


\paragraph{Air}
Atmospheric emissions shall be limited at the source and shall comply with the relevant technical provisions of the following regulations:

\begin{itemize}    
    \item \textit{Arrêté du 02 février 1998 relatif aux prélèvements et à la consommation d'eau ainsi qu'aux émissions de toute nature des installations classées pour la protection de l'environnement soumises à autorisation, Articles 26, 27, 28, 29, 30.}
\end{itemize}

\noindent The design of exhaust air discharge points shall comply with the requirements of the section 5.1.3 of the CERN Safety Guideline C-1-0-3 - Practical guide for users of Local exhaust ventilation (LEV) systems. 

\noindent Whenever greenhouse gases are used, relevant technical provisions contained in the following regulations apply:

\begin{itemize}    
    \item Regulation (EU) No 517/2014 of the European Parliament and of the Council of 16 April 2014 on fluorinated greenhouse gases and repealing Regulation (EC) No 842/2006;                       
    \item \textit{Code de l'environnement Livre V: Titre II (Art. R521-54 to R521-68) and Titre IV (Art. R543-75 to R543-123).}
\end{itemize}

\noindent All the appropriate preventive measures shall be taken against the release of greenhouse gases into the atmosphere. Working procedures shall be established and implemented for activities involving the use of those gases including the storage, handling, transport, recovery and disposal. Additionally such activities shall be performed by trained personnel. The emissions of fluorinated gases shall be registered during the entire life-cycle of the equipment or Experiment.

In accordance with the siting of the facility on French territory, the design, operation and maintenance of cooling tower water circuits shall comply with the relevant technical provisions of the following regulations and standards in order to limit the risk of legionella bacteria and its dispersion in the atmosphere:

\begin{itemize}    
    \item \textit{NF E38-424 Aéroréfrigérants humides : terminologie et exigences de conception vis-à-vis du risque légionellose;}                       
    \item \textit{Arrêté du 14 décembre 2013 relatif aux prescriptions générales applicables aux installations relevant du régime de l'enregistrement au titre de la rubrique no 2921 de la nomenclature des installations classées pour la protection de l'environnement;}
    \item \textit{Guide des bonnes pratiques Legionella et tours aéroréfrigérantes.}
\end{itemize}

\paragraph{Water}
The BDF project shall ensure the rational use of water. The discharge of effluent water into the CERN clean and sewage water networks shall comply with the relevant technical provisions contained in the following regulations:

\begin{itemize}    
    \item \textit{Loi n\si{\degree} 2006-1772 du 30 décembre 2006 sur l'eau et les milieux aquatiques;}                       
    \item \textit{Arrêté du 02 février 1998 relatif aux prélèvements et à la consommation d'eau ainsi qu'aux émissions de toute nature des installations classées pour la protection de l'environnement soumises à autorisation.}
\end{itemize}

\noindent The direct or indirect introduction of potentially polluting substances into water, including their infiltration into ground is prohibited. Applicable emission limit values for effluent water discharged in the Host States territory are defined in the following regulations:

\begin{itemize}    
    \item \textit{Arrêté du 02 février 1998 relatif aux prélèvements et à la consommation d'eau ainsi qu'aux émissions de toute nature des installations classées pour la protection de l'environnement soumises à autorisation Art. 31 and art.32.}
\end{itemize}

\noindent In complement, in case independent cooling towers are installed, the cooling circuit shall be equipped with a recycling process, and the effluent resulting from the recycling process shall be discharged into the sanitary network.

Retention measures for fire extinguishing water are required for any CERN project in which large quantities of hazardous, or potentially polluting substances are used or stored. As the project moves to the Technical Design Report stage, through discussions with the Environmental Protection specialists from HSE, it will be determined whether the following guidance document shall be applied (in accordance with the French \textit{Code de l'Environnement}:

\begin{itemize}    
    \item \textit{Référentiel APSAD D9 : Dimensionnement des besoins en eau pour la défense contre d'incendie and Référentiel APSAD D9A : Dimensionnement des rétentions des eaux d'extinction available in the Centre National de Prévention et de Protection (CNNP) (http://www.cnpp.com/).}
\end{itemize}


\paragraph{Energy}
The use of energy shall be done as efficiently as possible. For the entire facility, adequate measures shall be taken to comply with the relevant technical provisions contained in the following regulations:

\begin{itemize}    
    \item \textit{Loi no 2010-788 du 12 juillet 2010 portant engagement national pour l'environnement (Grenelle II).}
\end{itemize}

\noindent In addition, construction of new buildings sited in France shall comply with the relevant technical provisions relating to thermal efficiency contained in the following regulation:

\begin{itemize}
    \item \textit{Décret no 2012-1530 du 28 décembre 2012 relatif aux caractéristiques thermiques et à la performance énergétique des constructions de bâtiments.}
    \item \textit{Arrêté du 26 octobre 2010 relatif aux caractéristiques thermiques et aux exigences de performance énergétique des bâtiments nouveaux et des parties nouvelles de bâtiments and the French Réglementation Thermique 2012 (RT 2012).} 
    \item \textit{NF EN 15232 Performance énergétique des bâtiments - Impact de l'automatisation, de la régulation et de la gestion technique.} 
\end{itemize}

\paragraph{Soil}

The natural physical and chemical properties of the soil must be preserved. All the relevant technical provisions related to the usage and/or storage of hazardous substances to the environment shall be fulfilled to avoid any chemical damage on soil. Furthermore, the excavated material shall be handled adequately and prevent further site contamination. All excavated material must be disposed of appropriately in accordance with the associated waste regulations. 

\paragraph{Waste}

The selection of construction materials, design and fabrication methods shall be such that the generation of waste is both minimised and limited at the source. Waste shall be handled from its collection to its recovery or disposal according to: 

\begin{itemize}
    \item \textit{Code de l'environnement,  Livre V: Titre IV -Déchets ;}
    \item \textit{LOI no 2009-967 du 3 août 2009 de programmation relative à la mise en oeuvre du Grenelle de l'environnement (1), Art. 46;} 
\end{itemize}

\noindent The traceability of the waste shall be guaranteed at any time.

\paragraph{Preservation of the natural environment}

The BDF project shall ensure the preservation of the natural environment (e.g. landscaping, fauna, floral reserve, etc.) according to the relevant technical provisions contained in the following regulations:

\begin{itemize}    
    \item \textit{Code de l'environnement, Art. L411-1.}
\end{itemize}

\noindent Vegetal species listed in this regulation shall be protected, restored or adequately replaced (e.g. orchids). Whenever CERN natural areas are affected by a project, the Civil Engineering and Buildings (SMB-SE-CEB) section of the SMB Department shall be contacted for authorisation and definition of appropriate measures.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Transport and handling %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Transport and Handling}
\label{sec:ICE_Transport}

To be written by Ingo
